VicaSplat: A Single Run is All You Need for 3D Gaussian Splatting and Camera Estimation from Unposed Video Frames

We present VicaSplat, a novel framework for joint 3D Gaussians reconstruction and camera pose estimation from a sequence of unposed video frames, which is a critical yet underexplored task in real-world 3D applications. The core of our method lies in a novel transformer-based network architecture. In particular, our model starts with an image encoder that maps each image to a list of visual tokens. All visual tokens are concatenated with additional inserted learnable camera tokens. The obtained tokens then fully communicate with each other within a tailored transformer decoder. The camera tokens causally aggregate features from visual tokens of different views, and further modulate them frame-wisely to inject view-dependent features. 3D Gaussian splats and camera pose parameters can then be estimated via different prediction heads. Experiments show that VicaSplat surpasses baseline methods for multi-view inputs, and achieves comparable performance to prior two-view approaches. Remarkably, VicaSplat also demonstrates exceptional cross-dataset generalization capability on the ScanNet benchmark, achieving superior performance without any fine-tuning. Project page: https://lizhiqi49.github.io/VicaSplat.

==> tables/ablation_pose_align.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablations.} intrinsic embeddings are vital for performance and using intrinsic tokens performs the best. Adding the RGB image shortcut also improves the quality of rendered images. Our method achieves better performance compared with the pose-required per-local-view Gaussian field prediction method.
}
\begin{adjustbox}{max width=\linewidth}
\setlength{\tabcolsep}{0.08cm}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{ll ccc ccc}
\toprule
& & \multicolumn{3}{c}{Novel-view Synthesis} & \multicolumn{3}{c}{Pose Estimation} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
Num & Design & PSNR & SSIM & LPIPS & ATE & RPE trans & RPE rot \\
\midrule
(a) & Ours & \best{24.537} & \second{0.814} & \best{0.162} & \second{0.020} & 0.047 & \best{1.209} \\
\midrule
(b) & w/o framewise mod. & 21.655 & 0.706 & 0.222 & 0.026 & 0.060 & 1.616  \\
(c) & w/o CN-attn & 19.908 & 0.644 & 0.287 & 0.042 & 0.107 & 2.691 \\
(d) & full attn. for camera & 22.505 & 0.738 & 0.201 & 0.021 & 0.048 & \second{1.240} \\
(e) & w/o pose alignment & \second{22.514} & 0.738 & \best{0.197} & \best{0.019} & \best{0.045} & 1.264 \\
(f) & quat.+trans. for camera & 22.513 & \best{0.740} & \best{0.197} & \best{0.019} & \second{0.046} & 1.314 \\
% \midrule
% (g) & w/o rendering supervision & 24.632 & 0.834 & 0.167 & - & - & - \\
% (h) & w/o camera supervision & 24.632 & 0.834 & 0.167 & - & - & - \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:ablation}
\end{table}

==> tables/nvs_dl3dv.tex <==
\begin{table*}[!t]
    \centering
    \caption{\textbf{Novel view synthesis performance comparison on the DL3DV~\citep{dl3dv} dataset}. 
    Our method largely outperforms previous pose-free methods on all overlap settings, and even outperforms SOTA pose-required methods, especially when the overlap is small.}
    \begin{adjustbox}{max width=\textwidth}
    \setlength{\tabcolsep}{0.08cm}
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{llccc ccc ccc ccc}
        \toprule
        & & \multicolumn{3}{c}{2 views} & \multicolumn{3}{c}{4 views} & \multicolumn{3}{c}{8 views} & \multicolumn{3}{c}{16 views} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
        & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
        \midrule
        \multirow{4}{*}{\shortstack[l]{\emph{Pose-} \\ \emph{Required}}} 
        % & pixelNeRF & 18.417 & 0.601 & 0.526 & 19.930 & 0.632 & 0.480 & 20.869 & 0.639 & 0.458 & 19.824 & 0.626 & 0.485 \\
        & pixelSplat & - & - & - & - & - & - & - & - & - & - & - & - \\
        & MVSplat & - & - & - & - & - & - & - & - & - & - & - & - \\
        & FreeSplat & - & - & - & - & - & - & - & - & - & - & - & - \\
        \midrule
        \multirow{5}{*}{\shortstack[l]{\emph{Pose-} \\ \emph{Free}}} 
        & Splatt3R & - & - & - & - & - & - & - & - & - & - & - & - \\
        & NoPoSplat & - & - & - & - & - & - & - & - & - & - & - & - \\
        & CoPoNeRF & - & - & - & - & - & - & - & - & - & - & - & - \\
        & \best{Ours} & \best{-} & \best{-} & \best{-} & \best{-} & \best{-} & \best{-} & \best{-} & - & - & \best{-} & \best{-} & \best{-} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
\label{tab:dl3dv}
\end{table*}


==> tables/nvs_re10k.tex <==
\begin{table*}[!t]
    \centering
    \caption{\textbf{Novel view synthesis performance comparison on the RealEstate10k~\citep{re10k} dataset}. 
    Our method largely outperforms previous pose-free methods on all overlap settings, and even outperforms SOTA pose-required methods, especially when the overlap is small.}
    \begin{adjustbox}{max width=\textwidth}
    \setlength{\tabcolsep}{0.08cm}
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{llccc ccc ccc ccc}
        \toprule
        & & \multicolumn{3}{c}{2 views} & \multicolumn{3}{c}{4 views} & \multicolumn{3}{c}{8 views} & \multicolumn{3}{c}{16 views} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
        & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
        \midrule
        \multirow{3}{*}{\shortstack[l]{\emph{Pose-} \\ \emph{Required}}} 
        % & pixelNeRF & 18.417 & 0.601 & 0.526 & 19.930 & 0.632 & 0.480 & 20.869 & 0.639 & 0.458 & 19.824 & 0.626 & 0.485 \\
        & pixelSplat & 20.263 & 0.717 & 0.266 & 23.711 & 0.809 & 0.181 & 27.151 & 0.879 & 0.122 & 23.848 & 0.806 & 0.185 \\
        & MVSplat & 20.353 & 0.724 & 0.250 & 23.778 & 0.812 & 0.173 & 27.408 & \best{0.884} & \best{0.116} & 23.977 & 0.811 & 0.176 \\
        & FreeSplat & 19.151 & 0.663 & 0.368 & 22.532 & 0.763 & 0.269 & 25.897 & 0.845 & 0.186 & 22.664 & 0.762 & 0.269 \\
        \midrule
        \multirow{3}{*}{\shortstack[l]{\emph{Pose-} \\ \emph{Free}}} 
        % & Splatt3R & 14.352 & 0.475 & 0.472 & 15.529 & 0.502 & 0.425 & 15.817 & 0.483 & 0.421 & 15.318 & 0.490 & 0.436 \\
        & NoPoSplat & 14.101 & 0.432 & 0.468 & 15.419 & 0.451 & 0.432 & 16.427 & 0.453 & 0.402 & 15.382 & 0.447 & 0.432 \\
        & CoPoNeRF & 17.393 & 0.585 & 0.462 & 18.813 & 0.616 & 0.392 & 20.464 & 0.652 & 0.318 & 18.938 & 0.619 & 0.388 \\
        & \best{Ours} & \best{22.514} & \best{0.784} & \best{0.210} & \best{24.899} & \best{0.839} & \best{0.160} & \best{27.411} & 0.883 & 0.119 & \best{25.033} & \best{0.838} & \best{0.160} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
\label{tab:re10k}
\end{table*}


==> tables/nvs_re10k_2views.tex <==
\begin{table}[!t]
    \centering
    \caption{\textbf{Novel view synthesis performance comparison on the RealEstate10k~\citep{re10k} dataset under 2-views setup}. }
    \begin{adjustbox}{max width=\linewidth}
    \setlength{\tabcolsep}{0.08cm}
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{llccc ccc ccc ccc}
        \toprule
        & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
        \midrule
        \multirow{3}{*}{\shortstack[l]{\emph{Pose-} \\ \emph{Required}}} 
        % & pixelNeRF & 18.417 & 0.601 & 0.526 & 19.930 & 0.632 & 0.480 & 20.869 & 0.639 & 0.458 & 19.824 & 0.626 & 0.485 \\
        & pixelSplat~\cite{charatan2024pixelsplat} & - & - & - \\
        & MVSplat~\cite{chen2025mvsplat} & - & - & - \\
        & FreeSplat~\cite{wang2024freesplat} & - & - & - \\
        \midrule
        \multirow{3}{*}{\shortstack[l]{\emph{Pose-} \\ \emph{Free}}} 
        % & Splatt3R & 14.352 & 0.475 & 0.472 & 15.529 & 0.502 & 0.425 & 15.817 & 0.483 & 0.421 & 15.318 & 0.490 & 0.436 \\
        & NoPoSplat~\cite{ye2024noposplat} & - & - & - \\
        & CoPoNeRF~\cite{hong2024coponerf} & - & - & - \\
        & \best{Ours} & \best{20.824} & \best{0.664} & \best{0.239} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
\label{tab:re10k}
\end{table}


==> tables/nvs_re10k_dl3dv_multiview.tex <==
\begin{table*}[!t]
    \centering
    \caption{\textbf{Novel view synthesis performance comparison on the DL3DV~\citep{dl3dv} dataset}. 
    Our method largely outperforms previous pose-free methods on all overlap settings, and even outperforms SOTA pose-required methods, especially when the overlap is small.}
    \begin{adjustbox}{max width=\textwidth}
    \setlength{\tabcolsep}{0.08cm}
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{llccc ccc | ccc ccc}
        \toprule
        & & \multicolumn{3}{c}{4 views (RE10k)} & \multicolumn{3}{c}{8 views (RE10k)} & \multicolumn{3}{c}{4 views (DL3DV)} & \multicolumn{3}{c}{8 views (DL3DV)} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
        & Method & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
        \midrule
        \multirow{4}{*}{\shortstack[l]{\emph{Pose-} \\ \emph{Required}}} 
        % & pixelNeRF & 18.417 & 0.601 & 0.526 & 19.930 & 0.632 & 0.480 & 20.869 & 0.639 & 0.458 & 19.824 & 0.626 & 0.485 \\
        & pixelSplat & 24.836 & 0.838 & 0.160 & - & - & - & 20.220 & 0.706 & 0.265 & 20.734 & 0.682 & 0.253 \\
        & MVSplat & - & - & - & - & - & - & - & - & - & - & - & - \\
        & FreeSplat & 20.630 & 0.747 & 0.313 & 21.259 & 0.767 & 0.309 & 16.589 & 0.597 & 0.414 & 17.409 & 0.558 & 0.458 \\
        \midrule
        \multirow{5}{*}{\shortstack[l]{\emph{Pose-} \\ \emph{Free}}} 
        % & Splatt3R & - & - & - & - & - & - & - & - & - & - & - & - \\
        & NoPoSplat & - & - & - & - & - & - & - & - & - & - & - & - \\
        & CoPoNeRF & 18.299 & 0.655 & 0.559 & - & - & - & 17.942 & 0.650 & 0.594 & 18.515 & 0.655 & 0.592 \\
        & \best{Ours} & \best{-} & \best{-} & \best{-} & \best{-} & \best{-} & \best{-} & \best{-} & - & - & \best{-} & \best{-} & \best{-} \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
\label{tab:dl3dv}
\end{table*}


==> tables/pose.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Evaluation on Camera Pose Estimation} on RealEstate10k~\citep{re10k}, ACID~\cite{acid}, and ScanNet~\citep{scannet} datasets.
Our method achieves the best overall performance among all online methods.
}
% \footnotesize
\renewcommand{\arraystretch}{1.}
% \renewcommand{\tabcolsep}{2.5pt}
% \resizebox{\textwidth}{!}{
\begin{adjustbox}{max width=\textwidth}
\setlength{\tabcolsep}{0.08cm}
\begin{tabular}{@{}clccccc|ccc|ccc@{}}
\toprule
& & & & \multicolumn{3}{c}{\textbf{RE10k}} & \multicolumn{3}{c}{\textbf{ACID}} & \multicolumn{3}{c}{\textbf{ScanNet}} \\ 
\cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
{} & {Method}  &  \textbf{Optim.} & \textbf{Onl.} & {ATE $\downarrow$} & {RPE trans $\downarrow$} & {RPE rot $\downarrow$} & {ATE $\downarrow$} & {RPE trans $\downarrow$} & {RPE rot $\downarrow$} & {ATE $\downarrow$} & {RPE trans $\downarrow$} & {RPE rot $\downarrow$} \\ 
\midrule
 & VGGSFM~\cite{wang2024vggsfm} & \checkmark & & 0.141 & \textbf{0.035} & \underline{0.615} & \underline{0.071} & \textbf{0.010} & 1.712 & 0.158 & 0.034 & 1.618 \\ 
 & DUSt3R~\cite{wang2024dust3r} & \checkmark & & 0.417 & 0.250 & 5.796 & 0.083 & 0.017 & 3.567 & {0.081} & 0.028 & 0.784 \\  
{ }& MASt3R~\cite{leroy2025mast3r} & \checkmark & & {{0.185}} & {0.060} & {1.496} & {\bf{0.038}} & {\underline{0.012}} & {\bf{0.448}} & {\underline{0.078}} & {\underline{0.020}} & {\bf {0.475}} \\ 
& MonST3R~\cite{zhang2024monst3r}  & \checkmark & & \bf {{0.111}} & \underline{0.044} & {0.869} & {{0.098}} & {{0.019}} & {\underline{0.935}} & {\bf{0.077}} & {\bf{0.018}} & {\underline{0.529}} \\ 
& Spann3R~\cite{wang2024spann3r} & &\checkmark  & {{0.329}} & \underline{0.110} & \underline{4.471} & {\underline{0.056}} & {\underline{0.021}} & {\underline{0.591}} & {\bf{0.096}} & {\underline{0.023}} & {\underline{0.661}} \\ 

& Ours &  & \checkmark & \bf 0.213 & \bf 0.066 & \bf 0.621 & \textbf{0.046} & \bf 0.015 & \bf 0.473 & \underline{0.099} & \textbf{0.022} & \textbf{0.600}\\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-.1in}
\label{tab:pose}
\end{table*}

==> tables/training_config.tex <==
% lr, batch_size, n_iter, loss, n_target_views

\begin{table}[t]
\centering
\caption{\textbf{Configuration of different training stages.} }
\begin{adjustbox}{max width=\linewidth}
\setlength{\tabcolsep}{0.08cm}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{l|ccccc}
\toprule

Stage & lr & batch\_size & n\_iter & loss & n\_target\_views \\
\midrule
Point Distillation & 4e-5 & 192 & 10000 & $\mathcal{L}_{distill}$ & - \\
2-view & 2e-5 & 128 & 30000 & $\mathcal{L}_{img}+\mathcal{L}_{camera}$ & 4 \\
4-view & 1e-5 & 64 & 20000 & $\mathcal{L}_{img}+\mathcal{L}_{camera}$ & 6 \\
8-view & 1e-5 & 16 & 30000 & $\mathcal{L}_{img}+\mathcal{L}_{camera}$ & 12 \\
% \midrule
% (g) & w/o rendering supervision & 24.632 & 0.834 & 0.167 & - & - & - \\
% (h) & w/o camera supervision & 24.632 & 0.834 & 0.167 & - & - & - \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:training_config}
\end{table}
